Simulation of the abstract Tile Assembly Model Using Crisscross Slats

Tile assembly systems in the abstract Tile Assembly Model (aTAM) are computationally universal and capable of building complex shapes, but DNA-based implementations encounter formidable error rates that stifle this theoretical potential. Slat-based self-assembly is a recent development wherein DNA forms long slats that combine together in 2 layers, rather than the aTAM's square tiles in a plane. While tiles tend to bind to 2 neighboring tiles at a time, slats may bind to dozens of other slats. Large slat-based DNA constructions have been implemented in the lab with incredible resilience to many of the errors that plague tile-based constructions, but these come at a cost as slat-based systems are often more difficult to design and simulate. Also, it has not been clear if slats, with their larger sizes and different geometries, have the same theoretical capabilities as tiles. Here we show that slats do, at least at scale. We give constructions showing that any aTAM system may be simulated by a system of slats and that these can be made more efficiently, using shorter slats and a smaller scale factor, when simulating simpler classes of systems. We consider 5 classes of aTAM systems with increasing complexity, from zig-zag systems to the full class of all aTAM systems, and show how they can be converted to equivalent slat systems. Zig-zag systems can be simulated by slats at only a $2c \times 2c$ scale (where $c$ is the freely chosen cooperativity of the slats), the full class of aTAM systems at only a $5c \times 5c$ scale, and intermediate classes using scales between these. Together, these results prove that slats have the full theoretical power of aTAM tiles while providing constructions compact enough to potentially provide designs for DNA-based implementations of slat systems that are both capable of powerful algorithmic self-assembly and possessing the strong error resilience of slats.

==> aTAM-sim.tex <==
\subsection{Intrinsic simulation in the aTAM}\label{sec:aTAM-sim}

This section describes what it means for a TAS to intrinsically simulate another TAS. In the following definitions, it will be assumed that $\calT = (T, \sigma_\calT, \tau_\calT )$ is a TAS being simulated by another TAS $\calS = (S, \sigma_\calS, \tau_\calS)$. Furthermore, let $\mathbb{Z}_n$ be the set $\{0, 1, \ldots, n-1\}$ equipped with the typical notions of modular arithmetic. \todo{short informal explanation of scale factor, macrotiles, ...}

Given a positive integer $c$ called the \emph{scale factor}, a \emph{$c$-block macrotile} over $S$ is a partial function $\mu:\mathbb{Z}_c \dashrightarrow S$. That is, $\mu$ assigns tiles from $S$ to some subset of the locations in a $c\times c$ block of locations. If the domain of $\mu$ is empty, then the macrotile is called \emph{empty}. During a simulation, it is assumed that the lattice $\mathbb{Z}^2$ is divided regularly into $c$-block macrotiles so that the origin occupies the south-westernmost location in the corresponding macrotile block. Given a general assembly $\alpha \in \mathcal{A}^\calS$ and some coordinates $(x,y)\in \mathbb{Z}^2$, we can recover the macrotiles from $\alpha$ by letting $\mathcal{M}^c_{x,y}[\alpha]$ refer to the $c$-block macrotile in $\alpha$ whose southwest corner occupies location $(cx,cy)$. In other words $\mathcal{M}^c_{x,y}[\alpha](i,j) = \alpha(cx+i, cy+j)$, when defined, for $(i,j)\in\mathbb{Z}^2_c$.

\todo{representation functions and fuzz}

\begin{definition} \label{def:atam-sim-equiv-prod}
    We say that $\calS$ and $\calT$ have \emph{equivalent productions} (under $R$), written $\calS \Leftrightarrow_R \calT$, if the following conditions hold:
    \begin{itemize}
        \item $\{R^*(\alpha') | \alpha' \in \prodasm{\calS}\} = \prodasm{\calT}$,
        \item $\{R^*(\alpha') | \alpha' \in \termasm{\calS}\} = \termasm{\calT}$, and
        \item For all $\alpha'\in\prodasm{\calS}$, $\alpha'$ maps cleanly to $R^*(\alpha')$.
    \end{itemize}
\end{definition}

\begin{definition} \label{def:atam-sim-follows}
    We say that $\calT$ \emph{follows} $\calS$ (under $R$), written $\calT \dashv_R \calS$, if for all $\alpha', \beta' \in \prodasm{\calS}$, $\alpha' \to^\calS \beta'$ implies $R^*(\alpha') \to^\calT R^*(\beta')$.
\end{definition}

In the following definition let ${R^*}^{-1}(\alpha)$ refer to the producible pre-image of the assembly representation function $R^*$ on $\alpha$. That is ${R^*}^{-1}(\alpha) = \{\alpha' \in \prodasm{\calS} | R^*(\alpha') = \alpha \}$, so that ${R^*}^{-1}(\alpha)$ consists of all $\calS$-producible assemblies that represent $\alpha$ under $R$.

\begin{definition} \label{def:atam-sim-models}
    We say that $\calS$ \emph{models} $\calT$ (under $R$), written $\calS \vDash_R \calT$, if for every $\alpha \in \prodasm{\calT}$, there exists a non-empty subset $\Pi_\alpha \subseteq {R^*}^{-1}(\alpha)$, such that for all $\beta \in \prodasm{\calT}$ where $\alpha \to^\calT \beta$, the following conditions are satisfied:
    \begin{enumerate}
        \item for every $\alpha' \in \Pi_\alpha$, there exists $\beta' \in {R^*}^{-1}(\beta)$ such that $\alpha' \to^\calS \beta'$
        \item for every $\alpha''\in {R^*}^{-1}(\alpha)$ and $\beta''\in {R^*}^{-1}(\beta)$ where $\alpha'' \to^\calS \beta''$, there exists $\alpha'\in \Pi_\alpha$ such that $\alpha' \to^\calS \alpha''$.
    \end{enumerate}
\end{definition}

In Definition~\ref{def:atam-sim-models} above, the set $\Pi_\alpha$ is defined to be a set of assemblies representing $\alpha$ from which it is still possible to produce assemblies representing all possible $\beta$ producible from $\alpha$. Informally, the first condition specifies that all assemblies in $\Pi_\alpha$ can produce some assembly representing any $\beta$ producible from $\alpha$, while the second condition specifies that any assembly $\alpha''$ representing $\alpha$ that may produce an assembly representing $\beta$ is producible from an assembly in $\Pi_\alpha$. In this way, $\Pi_\alpha$ represents a set of the earliest possible representations of $\alpha$ where no commitment has yet been made regarding the next simulated assembly. Requiring the existence of such a set $\Pi_\alpha$ for every producible $\alpha$ ensures that non-determinism is faithfully simulated. That is, the simulation cannot simply ``decide in advance'' which tile attachments will occur.\todo{This paragraph is duplicated from the section defining aSAM simulation of aTAM. Maybe that could be noted or it could be removed.}
